DeepCC: Bridging the Gap Between Congestion Control and Applications via Multi-Objective Optimization

The increasingly complicated and diverse applications have distinct network performance demands, e.g., some desire high throughput while others require low latency. Traditional congestion controls (CC) have no perception of these demands. Consequently, literatures have explored the objective-specific algorithms, which are based on either offline training or online learning, to adapt to certain application demands. However, once generated, such algorithms are tailored to a specific performance objective function. Newly emerged performance demands in a changeable network environment require either expensive retraining (in the case of offline training), or manually redesigning a new objective function (in the case of online learning). To address this problem, we propose a novel architecture, DeepCC. It generates a CC agent that is generically applicable to a wide range of application requirements and network conditions. The key idea of DeepCC is to leverage both offline deep reinforcement learning and online fine-tuning. In the offline phase, instead of training towards a specific objective function, DeepCC trains its deep neural network model using multi-objective optimization. With the trained model, DeepCC offers near Pareto optimal policies w.r.t different user-specified trade-offs between throughput, delay, and loss rate without any redesigning or retraining. In addition, a quick online fine-tuning phase further helps DeepCC achieve the application-specific demands under dynamic network conditions. The simulation and real-world experiments show that DeepCC outperforms state-of-the-art schemes in a wide range of settings. DeepCC gains a higher target completion ratio of application requirements up to 67.4% than that of other schemes, even in an untrained environment.

==> Evaluation.tex <==

% \begin{figure}[t]
% 	\centerline{\includegraphics[width=0.70\linewidth]{figures/goal_tuning_time.pdf}}
% 	\vspace{-0.15in}
% 	\caption{\label{fig:goal_tuning}Online decision interval.}
% 	% \label{single-scenario-multi-objective}
% 	\vspace{-0.25in}
% \end{figure}
\section{Evaluation}
	\label{sec:evaluation}
	In this section, we first present the overhead and the decision interval. Then we evaluate the main properties of DeepCC and compare it with the state-of-the-art schemes through emulator, including multi-objective optimization, online tuning, convergence and robustness. We also show the results of competing among DeepCC or non-DeepCC flows on our testbed. Finally, we evaluate DeepCC in the wild. 
	\begin{figure*}[t]
        \centering
        % \vspace{-0.15in}	
        \subfigure[Offline performance over Wi-Fi link]{
            \label{Dynamic-offline} %% label for first subfigure
            \includegraphics[width=0.32\linewidth]{figures/dynamic-offline.pdf}}
        % \hspace{0.8in}
        \hspace{0.01in}
        % \vspace{-0.1in}	
        \subfigure[Offline performance over cellular link]{
            \label{LTE-offline} %% label for second subfigure
            \includegraphics[width=0.315\linewidth]{figures/ATT-offline.pdf}}
        \hspace{0.01in}	
        \subfigure[Online performance over cellular link]{
            \label{ATT-online} %% label for second subfigure
            \includegraphics[width=0.22\textheight]{figures/ATT-online-icnp.pdf}}
    % 		\hspace{-0.1in}	
        % \vspace{-0.1in}
        \caption{Performance frontier achieved by DeepCC. The color bar represents the packet loss rate where darker is worse. }
        \label{offline-fig} % % label for entire figure	
        % \vspace{-0.15in}	
    \end{figure*} 
% 	to reduce the throughput degradation and the delay jitter.
% \vspace{-0.05in}
\begin{table*}[!tbh]
	\renewcommand\arraystretch{1.0}
	\centering
	\caption{The completion ratio of online tuning algorithm with 500 random target values.}\label{online-table}
	% \vspace{-0.1in}
	\scalebox{0.99}[0.95]{
	  %  \small
		\begin{tabular}{@{}cccc|cccc@{}}
		\toprule
		& \multicolumn{3}{c|}{Wi-Fi Network}         & & \multicolumn{3}{c}{Cellular Network}        \\ 
		&CR(\%)  & CR(\%)&CR(\%)
		&& CR(\%)& CR(\%)& CR(\%)\\ 
		Scheme& (error$=0\%$)& (error$<5\%$)& (error$<10\%$)            
		&Scheme& (error$=0\%$)& (error$<5\%$)& (error$<10\%$)\\ 
		\midrule
		Cubic &  0.0  & 0.0   & 0.0 & Cubic &  0.0  & 0.2 &  3.0 \\ BBR &  0.2   &  11.4   &  21.8 & BBR & 0.0 & 0.0 & 0.0  \\
		Remy($\delta= 0.1$)&  43.0  & 45.2   & 47.4    &Remy($\delta= 0.1$)&   44.2  &  47.4   &  49.8    \\
		Remy($\delta=1.0$)&  34.4  & 37.2   & 39.0     & Remy($\delta=1.0$)&   15.2  &  15.4  &  16.0    \\
		Remy($\delta=10$)&  41.4  & 44.0   & 45.8     &  Remy($\delta=10$)&   12.2  &  13.6   &  14.2     \\
		PCC-Allegro&  42.8  & 46.8   & 51.4     & PCC-Allegro&   0.0 & 0.0 & 0.0      \\	
		Vivace-latency&  63.4  & 65.6   & 71.0    & Vivace-latency&    0.0  &   0.0   &   0.0          \\
		Vivace-loss&   0.0  &  0.0   &  0.0     & Vivace-loss&    0.0  &   0.0   &   0.0         \\
		Vivace-LTE&  64.6  & 70.6   & 77.4    & Vivace-LTE&   0.0 & 0.0 & 0.0         \\
		Indigo&  3.0  & 3.2   & 4.2    & Indigo&   3.2  &  3.8   &  4.0          \\
		\textbf{DeepCC} &  \textbf{88.8}  & \textbf{93.6}   & \textbf{95.8}    & \textbf{DeepCC}&   \textbf{67.4}  &  \textbf{71.4}   &  \textbf{75.4}         \\
		\bottomrule
		\end{tabular}
		}
	% \vspace{-0.25in}
\end{table*}

\subsection{Overhead and decision interval}
\label{eval:overhead}
DeepCC agent is trained on a PC with an Intel Core (TM) i7-6850k 3.6 GHz with 8 GB memory. It requires approximately two million training iterations to obtain the near Pareto optimal policies that perform well enough. In total, the training process took about 15 hours. 
In DeepCC, it takes about 0.9 ms on average to get the \emph{action} (i.e., the model inference time) or update the \emph{goal}. 
We carefully set the decision interval of the agent as 1/2 minimum RTT. Benefiting from that, the state can reflect the changes in network conditions in time. Meanwhile, it provides sufficient time for the action to be fully executed in the case of no congestion, which means the data sent by the sender can reach the receiver, thereby the estimation of reward is more accurate. Similarly, the online goal tuning is triggered by four RTTs rather than every ACK  according to our experimental results\footnote{We evaluate the online goal tuning module with different decision intervals from half to eight RTTs. The result shows that tuning triggered with four RTTs achieves the best performance. We omit the results due to space limitations.}.

    
\subsection{Dynamic behavior over multi-objective optimization}
	\label{offline-evaluation}
		To validate the effectiveness of multi-objective optimization, we repeatedly run DeepCC under two network scenarios with different {\em{goals}} in a broad range. Among them, we select 5 representative results, which are in the mode of high throughput, low delay, or the trade-offs. 
% 		We also compare DeepCC with not only PCC, Vivace, Remy and Indigo with their corresponding objective functions, but Linux kernel implementation schemes i.e., Cubic and BBR. 
		We also compared DeepCC with the off-the-shelf schemes. As shown in Fig.~\ref{Dynamic-offline} and (b), we intuitively visualize the performance of different schemes in a 2D throughput-delay space. The corresponding loss rate is shown via the color filled. 
		% The detailed observations are analyzed as follows. 
	
		\noindent \textbf{Emulated {Wi-Fi} link.}
		First, we test DeepCC over an emulated {Wi-Fi} link (from Pantheon~\cite{Francis2018Pantheon}) with high bandwidth variations, which DeepCC has been trained on. The link has an average 2.64 Mbps bandwidth following Poisson distribution, 176 ms minimum RTT and a drop-tail queue with 130 packets of buffer. As shown in Fig.~\ref{Dynamic-offline}, DeepCC with 5 representative goals achieves an efficient frontier that covers a wide range of trade-offs between throughput, queueing delay, and loss rate.

		Specifically, DeepCC with $g_{1}$ in high-throughput mode achieves comparable throughput with the state-of-the-art CCs, while reduces the queueing delay by up to 75\% with almost zero packet loss than them respectively. When running in the low-latency mode, DeepCC with $g_{5}$ performs almost the same as Remy. Other trade-off points stand in the middle and attain different trade-offs. These results show the efficiency of our multi-objective optimization.
		So DeepCC can achieve a large range of accessible trade-offs only by tuning the goal without any retraining or redesigning efforts and it achieves almost zero packet loss without sacrificing other performance metrics due to the high penalty of loss rate in the reward function.

		\noindent \textbf{Emulated cellular link.}
		To evaluate the performance of DeepCC in an unseen network link, we replay the AT\&T driving trace provided by~\cite{Winstein2013Stochastic}. The cellular link has 200 ms minimum RTT and 140 packets of buffer. As shown in Fig.~\ref{LTE-offline}, the performance of DeepCC with different goals also achieves an efficient frontier. 
		This results indicates that through training DeepCC has learned an adaptive policy supporting multi-objective optimization. However, to achieve a similar relative position of Fig.~\ref{Dynamic-offline}, DeepCC may require different goals. This phenomenon exposes the challenge on how to set the proper goal according to the network condition, which will be described in the following with our online tuning algorithm.
% 		But the generalization ability to adapt to different network conditions cannot be fully guaranteed when DeepCC only involves offline training.
\begin{figure*}[htbp]
	\begin{minipage}[t]{0.48\linewidth}
		\centering
		\includegraphics[width=0.98\textwidth]{figures/evaluation-convergence.pdf}
		% \vspace{-0.15in}
		\caption{\label{convergence time}Convergence time with different schemes.}
		% \vspace{-0.25in}
	\end{minipage}
	\hfill
	% \hspace{-0.01in}
	\begin{minipage}[t]{0.48\linewidth}
		\centering
		\includegraphics[width=0.9\textwidth]{figures/packet-loss.pdf}
		% \vspace{-0.15in}
		\caption{\label{packets-loss}Robustness to stochastic packet loss.}
	\end{minipage}
	\hfill
	% \begin{minipage}[t]{0.3\linewidth}
	% 	\centering
	% 	\includegraphics[width=0.75\textwidth]{figures/testbed-topology.pdf}
	% 	\vspace{-0.15in}
	% 	\caption{\label{fig:topology}Topology setup.}
	% \end{minipage}
	% \vspace{-0.25in}
\end{figure*}	

\subsection{Online performance}
	\label{online-evaluation}
	To investigate the generalization ability of DeepCC in online tuning, we randomly sample 500 target values $M$ of application requirements over above-mentioned {Wi-Fi} link and cellular link. The range of these target values $M$ is selected as follows: $M^{(1)}$ ranges from 0 to the achievable maximum throughput of all {learning}-based schemes on the corresponding link; $M^{(2)}$ varies from 0 to the achieved maximum queueing delay of all schemes on the corresponding link; and $M^{(3)}$, representing the loss rate, ranges from 0 to 10\%. Obviously, some of them can be achieved by none of the existing schemes. 
	
	Here, we denote the \emph{completion ratio (CR) (error$<=X\%$)} as the ratio of target achieved to all targets as our quantitative evaluation metric, where $X\%$ represents the acceptable relative error of performance when calculating the number of target achieved. Intuitively, for a given congestion control scheme, the higher completion ratio is obtained, the more application requirements can be achieved. Since all the existing learning-based schemes lack tunable objectives, we test each scheme with its default objective under the given network link and calculate its completion ratio. For DeepCC, we test it with different targets and leave the agent unchanged. 
	The results are shown in Table \ref{online-table}.
	As expected, DeepCC achieves the highest completion ratio than other schemes. Even in an untrained network scenario, DeepCC still achieves 67.4\% completion ratio, which could cover more if the constraint of acceptable error relaxes. The results indicate that through online tuning DeepCC can tune the objective to adapt to both network conditions and application requirements.
	
	As shown in Fig.~\ref{ATT-online}, the performance of DeepCC gains an efficient frontier again in the online stage. Compared with the frontier achieved by offline learning shown in Fig.~\ref{LTE-offline}, DeepCC with online tuning achieves a wider frontier than purely through offline learning. That is because DeepCC takes advantage of both offline and online learning. 
    When running online, it can timely regulate the near-optimal policy based on the offline trained agent according to the real-time network conditions.
	To provide a zoom-in view of online tuning, we select four targets and the corresponding achieved performance. 
	% Some of the targets are achievable while some are not.
    As shown, DeepCC tries to achieve the performance close to the frontier even if the target is unreachable.
% 	\begin{figure}[tb]
% 		\centerline{\includegraphics[width=0.9\linewidth]{figures/evaluation-convergence.pdf}}
% 		\vspace{-0.15in}
% 		\caption{\label{convergence time}Convergence time with different schemes.}
% 			% \label{single-scenario-multi-objective}
% 		\vspace{-0.25in}
% 	\end{figure}

% 	\begin{figure}[t]
% 		\centerline{\includegraphics[width=0.88\linewidth]{figures/packet-loss.pdf}}
% 		\vspace{-0.15in}
% 		\caption{\label{packets-loss}Robustness to stochastic packet loss.}
% 		% \label{single-scenario-multi-objective}
% 		\vspace{-0.25in}
% \end{figure}
% \begin{figure*}[htbp]
% 	\begin{minipage}[t]{0.48\linewidth}
% 		\centering
% 		\includegraphics[width=0.8\textwidth]{figures/fairness_same_tar.pdf}
% 		\vspace{-0.1in}
% 		\caption{\label{fig:fair-same-tar}Dynamic behavior of DeepCC flows with same targets.}
% 		\vspace{-0.25in}
% 	\end{minipage}
% 	\hfill
% 	% \hspace{-0.01in}
% 	\begin{minipage}[t]{0.48\linewidth}
% 		\centering
% 		\includegraphics[width=0.8\textwidth]{figures/diff_tar_tput.pdf}
% 		\vspace{-0.1in}
% 		\caption{\label{fig:diff-tar-tput}Throughput and delay of DeepCC flows with different targets.}
% 	\end{minipage}
% 	\hfill
% 	\vspace{-0.25in}
% \end{figure*}	

% \begin{figure}[t]
% 	\centerline{\includegraphics[width=0.70\linewidth]{figures/testbed-topology.pdf}}
% 	\vspace{-0.15in}
% 	\caption{\label{fig:topology}Topology setup.}
% 	% \label{single-scenario-multi-objective}
% 	\vspace{-0.25in}
% \end{figure}

\subsection{Convergence and robustness}

	\label{common properties}
		In the following, we evaluate the convergence and robustness of DeepCC. The emulated network link is set as a steady link with 12 Mbps, 60 ms RTT, and 90 KB of buffer. 

		\noindent\textbf{Convergence time.}
		\label{convergence-time}
		Although online schemes could react timely to the variable network conditions, the performance may be greatly impacted by convergence time. To evaluate DeepCC, we set the \emph{target} value $M$ as 12 Mbps throughput, 100 ms maximum delay, and 1\% loss rate. Fig.~\ref{convergence time} illustrates the convergence process of several congestion control schemes with 0.5s granularity. As the results showed, DeepCC has similar stable convergence behavior as the offline algorithms, i.e., Indigo and Remy (ver. $\delta$=1.0), but the throughput of DeepCC is higher than that of them. Compared with online learning schemes, DeepCC has the same ability to quickly lift throughput to 12 Mbps as Vivace (ver. latency), but the throughput of DeepCC oscillates less than that of it. In contrast, PCC takes the longest time to reach the throughput ceiling. Benefiting from offline and online learning, DeepCC gains a good start point from offline training and quickly adapts to network conditions through online fine-tuning. 

		\noindent\textbf{Robustness to packet loss.}
		When facing the lossy network condition, the loss-based and delay-based schemes often perform poorly, which is often shown as a sharp decline in throughput. On the contrary, the learning-based schemes can combat more non-congested packet loss since they do not take packet loss or delay as the explicit congestion signal.
			 
		To evaluate the robustness to packet loss of DeepCC, we set up a steady link with a stochastic loss rate ranging from 0\% to 6\%. The target for DeepCC is set as 11 Mbps throughput, 100 ms delay, and 5\% loss rate. The target loss rate represents the maximum tolerable link loss rate. 
		As shown in Fig.~\ref{packets-loss}, Remy is insensitive to packets loss, whereas it only achieves low throughput. PCC maintains throughput until the packet loss rate reaches 5\%, i.e., the predefined loss tolerance included in its objective function. The throughput of Vivace gradually decreases as the stochastic loss rate increases. 
		
		DeepCC remains insensitive to random packet loss and obtains consistent high throughput. This is because the goal (more precisely $g^{(3)}$) is not updated by the online tuning algorithm when the observed loss rate is less than that of target. Thus DeepCC ignores the random loss and runs to pursue the other two dimensions of the target (i.e., throughput and delay). If the observed loss rate is higher than that of target and the other two dimensions of measurement are satisfied with the target, DeepCC does not update the gradient according to the constraint of loss rate gradient in the online tuning algorithm. 
		
	
% 		\noindent\textbf{Fairness:}
% 		\label{Evaluation-fairness}
% 		To demonstrate the intra-protocol fairness of DeepCC, we set up the steady link sharing by three competing flows. The experiments last for 60 seconds with 3 flows starting sequentially with a 10-second interval. According to our above experiments, Remy is the most stable algorithm among the existing objective-based schemes. Thus we only compare DeepCC with Remy in this subsection.
% 		Fig.~\ref{fairness} shows the sending rate convergence process of each scheme with the granularity of 1 second. The results demonstrate that DeepCC with the same objective function (i.e., $g=(0.8,0.1,0.1)$) achieves the similar fairness to Remy. In addition, DeepCC has more stable convergence among competing flows than Remy when a new flow arrives. 


% 		\begin{figure}[t]
% 			\centering
% 			\subfigure
% 			{
% 				\includegraphics[width=0.45\linewidth, angle=0]{../figures/Fairness-DeepCC.pdf}
% 			}
% 			\subfigure
% 			{
% 				\includegraphics[width=0.45\linewidth, angle=0]{../figures/Fairness-Remy.pdf}
% 			}	
% 			\vspace{-0.13in}
% 			\caption{Intra-protocol fairness of DeepCC and Remy.}
% 			\label{fairness}
% 			\vspace{-0.15in}
% 		\end{figure}

\begin{figure}[t]
	\centerline{\includegraphics[width=0.95\linewidth]{figures/fairness_same_tar.pdf}}
	% \vspace{-0.15in}
	\caption{\label{fig:fair-same-tar}Dynamic behavior of DeepCC flows with the same target.}
	% \label{single-scenario-multi-objective}
	% \vspace{-0.25in}
\end{figure}

% \begin{figure}[t]
% 		\centerline{\includegraphics[width=0.75\linewidth]{figures/diff_tar_tput.pdf}}
% 		\vspace{-0.15in}
% 		\caption{\label{fig:diff-tar-tput}Throughput and delay of DeepCC flows with different targets.}
% 		\vspace{-0.25in}
% \end{figure}

\begin{figure*}[htbp]
	% \vspace{-0.1in}
	\begin{minipage}[t]{0.49\linewidth}
		\centering
		\includegraphics[width=0.75\linewidth]{figures/friendly.pdf}
		% \vspace{-0.15in}
		\caption{\label{fig:friendly}Throughput of different DeepCCs vs. Cubic.}
		% \vspace{-0.25in}
	\end{minipage}
	\hfill
	% \hspace{-0.01in}
	\begin{minipage}[t]{0.49\linewidth}
		\centering
		\includegraphics[width=0.85\linewidth]{figures/realworld-new.pdf}
		% \vspace{-0.15in}
		\caption{\label{fig-wild}Average throughput vs. delay in the wild. }
		% All schemes are repeatedly tested 10 times in different time periods. }
	\end{minipage}
	\hfill
	% \vspace{-0.25in}
\end{figure*}	

\subsection{Coexistence of DeepCC and non-DeepCC flows}
	\label{eval:fairness}
	To evaluate DeepCC with competing flows, we set up our testbed to experiment with the coexistence of DeepCC or non-DeepCC flows. We use two hosts as the sender and receiver respectively. They are connected through a router running OpenWrt. We use tc\cite{TC} in OpenWrt to regulate the bottleneck link with 10 Mbps bandwidth, 100 ms minimum RTT, and 120 KB of buffer. 
	% Bottleneck router buffer size is set to the BDP. 
	% In this section, we experimentally show the dynamic behavior among DeepCC and non-DeepCC flows. 
	
	\noindent\textbf{Coexistence of DeepCC flows with the same target.}
	To understand how DeepCC behaves as flows arrive and leave, we set up two competing flows with the same target, e.g., 10 Mbps high-throughput target. Fig. \ref{fig:fair-same-tar} shows the rate convergence process of DeepCC. The data transmission of the two flows initiates sequentially with a 100s interval and each flow transmits continuously for 500s. We can see that DeepCC flows with the same target converge to a similar throughput via the continuously \emph{goal} tuning. 
	
	% \noindent\textbf{Coexistence of DeepCC flows with different targets.}
	% A potential concern for DeepCC is how high-throughput flows affect the low-latency flows. We experiment on a bottleneck link with 10 Mbps bandwidth, 100 ms minimum RTT and 10 KB buffer size\cite{RouterBuffer}. 
	% Fig. \ref{fig:diff-tar-tput} shows the results. The performance of different flows achieves a similar throughput and delay respectively. Specifically, the queueing delay is only several milliseconds. Due to the shallow-buffered network, the controllable space of DeepCC is narrow. Under this circumstance, DeepCC would tune to a similar policy even facing different requirements, which degenerates from the multi-objective to the single-objective optimization.
	% However, these results can not fully reflect the performance of DeepCC in the real networks since the last mile is typically the speed bottleneck in communication networks\cite{lastMile}. Therefore, DeepCC can benefit from different bottlenecks to satisfy different targets \S\ref{eval:wild}. 
			
	% \begin{figure}[t]
	% 	\centerline{\includegraphics[width=0.80\linewidth]{figures/diff_tar_delay.pdf}}
	% 	\vspace{-0.1in}
	% 	\caption{\label{fig:diff-tar-delay}The delay of competing DeepCC flows under the different bottleneck-link buffer.}
	% 	% \label{single-scenario-multi-objective}
	% 	\vspace{-0.2in}
	% \end{figure}	

	% \begin{figure}[t]
	% 	\centerline{\includegraphics[width=0.80\linewidth]{figures/diff-bottleneck-topology.pdf}}
	% 	\vspace{-0.1in}
	% 	\caption{\label{fig:diff-bottleneck-topology}topology setup.}
	% 	% \label{single-scenario-multi-objective}
	% 	\vspace{-0.2in}
	% \end{figure}	
	

\noindent\textbf{Coexistence with non-DeepCC flows.}
	\label{eval:friendly}
	We evaluate DeepCC flows competing with Cubic flows on our testbed. We report the average throughput achieved by each flow of DeepCC and Cubic. Fig. \ref{fig:friendly} shows that the strong preemption of DeepCC in high-throughput mode benefits from the ability of utilizing the capacity of the bottleneck. It has a higher throughput than that of Cubic. When the target is in the low-latency mode, DeepCC has a weaker preemption of available bandwidth than that of Cubic. When the target is set in the middle, DeepCC achieves a better friendliness with competing Cubic flows.

	% \begin{figure}[t]
	% 	\centerline{\includegraphics[width=0.70\linewidth]{figures/friendly.pdf}}
	% 	\vspace{-0.15in}
	% 	\caption{\label{fig:friendly}Throughput of different DeepCCs versus Cubic.}
	% 	% \label{single-scenario-multi-objective}
	% 	\vspace{-0.18in}
	% \end{figure}
	% \begin{figure}[t]
	% 	\centerline{\includegraphics[width=0.8\linewidth]{figures/realworld-new.pdf}}
	% 	\vspace{-0.15in}
	% 	\caption{\label{fig-wild}Average throughput vs. 95th delay in the wild. All schemes are repeatedly tested 10 times in different time periods. }
	% 	\vspace{-0.25in}
	% \end{figure}
% \subsection{Online decision-interval}

% 	\begin{figure}[t]
% 		\centerline{\includegraphics[width=0.80\linewidth]{figures/goal_tuning_time.pdf}}
% 		\vspace{-0.1in}
% 		\caption{\label{fig:online-decision}The performance of different online decision makings.}
% 		% \label{single-scenario-multi-objective}
% 		\vspace{-0.2in}
% 	\end{figure}	

\subsection{Evaluation in the wild}
    % \vspace{-0.2in}
    \label{eval:wild}
	% We evaluate DeepCC in a realistic environment. The sender is deployed in Aliyun\cite{aliyun}. The receiver is located inside our campus and connected to the sender through the wide-area network. To validate the efficiency of DeepCC, we use tc\cite{TC} to add extra 62 KB buffer on this path (See \S\ref{discussion}). The resulting average bandwidth and minimum RTT of this path are 0.5 Mbps and 107 ms respectively.
	
	We evaluate DeepCC over wide-area Internet paths spanning two continents.
	%  from Asia to America. 
	The receiver is deployed in Amazon\cite{amazon} cloud. The sender is located inside our campus and connected to the receiver through the wide-area network.
	% We evaluate DeepCC under three \emph{goals} by only using the offline-learned agent. Further, 
	We evaluate DeepCC with three \emph{targets} and compare them against Cubic and BBR.
	The results are shown in Fig. \ref{fig-wild}. The average throughput and 95th percentile delay achieved by DeepCC are significantly different with three requirements. Guided by the \emph{target} value, DeepCC can not only satisfy the corresponding requirement but achieve better performance in both throughput and delay. The three targets of DeepCC achieve significantly lower delay than that of Cubic and BBR. Notice that BBR and high-throughput DeepCC are not sensitive to packets loss, they do well on throughput, but high-throughput DeepCC achieves lower delay than that of BBR. Cubic is sensitive to packet loss and hence loses throughput. 
	
	

	

    
 
